Reinforcement Learning for Economic Policy: A New Frontier?

Agent-based computational economics is a field with a rich academic history, yet one which has struggled to enter mainstream policy design toolboxes, plagued by the challenges associated with representing a complex and dynamic reality. The field of Reinforcement Learning (RL), too, has a rich history, and has recently been at the centre of several exponential developments. Modern RL implementations have been able to achieve unprecedented levels of sophistication, handling previously unthinkable degrees of complexity. This review surveys the historical barriers of classical agent-based techniques in economic modelling, and contemplates whether recent developments in RL can overcome any of them.

==> temp.tex <==
\section{Case Studies\label{sect:case-studies}}
This brief section hopes to extend the backdrop painted by the past two sections, with four contextual case studies of RL actually being incorporated in agent-based simulations, in economic settings. Through these examples, the core takeaway of the review---that RL can assist in the regard of agent-based representations---is affirmed.

\subsection{Modelling Dynamic Pricing Environments}
The first case study involves the idea of \emph{dynamic} pricing in markets. Kutschinski et al.~\cite{kutschinski2003learning} explored this idea almost two decades ago when they created the DMarks II platform---a multi-agent RL algorithm that could learn various strategic bidding and selling approaches in electronic marketplaces.

A recent application of this concept is in dynamic electricity pricing scenarios. Radhakrishnan et al.~\cite{Radhakrishnan2015} incorporated an RL algorithm in an ACE model of an electricity market, with an array of complex actors: a multitude of generation companies, many consumers with varying price caps, wholesale market traders, etc. Using this approach, the authors were able to achieve higher simulated incomes across all generating companies, when compared to the extant pricing models, by mapping supply to demand in a more efficient way. Ghasemi et al.~\cite{Ghasemi2020} extended these ideas to a `prosumer' microgrid model---where grid participants can both consume and produce, and thus can feed excess supply back into the grid, thereby generating revenue for themselves. Once again leveraging RL in an agent-based scenario, the authors were able to both reduce the overall grid costs, while simultaneously improving the net economic benefits for \emph{all} prosumers in the model.

Here we see examples of RL unlocking optimal multi-actor pricing strategies that would be very difficult to solve analytically. We can see that the general agent-based modelling philosophy remains, but the ability for actors to \emph{learn} is crucial for success.

\subsection{Modelling Adaptive Incentive Scenarios}
Rooted in Game Theory, ``Adaptive Incentive Design'' has recently been considered as a use case for RL-based simulations. The core of the problem is the so-called ``principal-agent'' relationship~\cite{ratliff2020adaptive}, where a ``principal'' actor aims to create an incentive policy that co-ordinates the agents in a simulation towards some overall minimized cost. Often, however, there exists an ``information asymmetry'' between the principal and the agents, leading to inefficiencies, which makes it a challenging problem to optimise.

Analytical solutions have been designed for certain scenarios, as is done by Ratliff and Fiez~\cite{ratliff2020adaptive}, but such approaches face limitations in the complexity they can handle. Yang et al.~\cite{yang2022}, in contrast, propose an RL-based solution, built around an agent-based model. In the paper itself, the authors focus on creating an optimal tax policy---as a special case of the principal-agent problem, where the principal is the tax-collecting entity, the agents are the tax payers, and `optimal' refers to some balance between proxies for equality and productivity. Nonetheless, their framework is sufficiently generic to cover a wide array of Adaptive Incentive problems. By adopting an RL approach, their proposed methods were able to learn near-optimal co-operative behaviour, despite starting with completely selfish agents, thus resulting in tax policies that beat the benchmarks for the aforementioned economic proxies. Similar work has been done by Zheng at al.~\cite{zheng2020ai} for RL-based tax policy, in creating the so-called ``AI-economist''. Outside of tax policy but relevant to this case study, Castro et al.~\cite{castro2020estimating} have proposed using RL in the context of liquidity allocation for banks operating in high-value payments systems. They too find that RL is able to learn optimal policies that minimise the costs for each individual agent, yielding benefit for all participants.

Tax policies, and these principal-agent problems more generally, are difficult to handle, for the competing interests and constraints they involve~\cite{zheng2020ai}. Nonetheless, these works---albeit nascent---indicate that RL-based implementations, via agent-based learning, can indeed find reasonably-optimal solutions, suggesting a potentially-bright future. Moreover, we see again that an approach involving hard-coded agents would likely struggle to capture the complex dynamics required for optimality---thereby affirming the necessity for \emph{learning} in the agents.

\subsection{Modelling Fiscal Policy}
Researchers have also looked at an adaptive-agent approach for macroeconomic modelling, with the goal of making fiscal and monetary policy decisions. An example is work by Hinterlang and Tänzer~\cite{hinterlang2021optimal}, who use RL to compute optimal interest rates to fulfill targeted inflation values. Using historical data from the United States, they find that the computed policy functions outperform traditional strategies, as well as the actual federal rates used at the time. These authors note how RL is able to capture the non-linear nature of complex economic models, which gives it great modelling flexibility, while not needing to know the full dynamics of the underlying environment. Chen et al.~\cite{chen2021deep} pursue a similar study, and arrive at the same conclusions.

\subsection{Modelling Sequential Social Dilemmas}
The fourth and final case study considered here is linked to the second, and is also rooted in Game Theory: the problem of ``Sequential Social Dilemmas.'' Such challenges manifest in a variety of ways, many of which indeed affect economic policy design. Social Dilemmas themselves have been studied for many years, with the most famous being the so-called ``Prisoner's Dilemma''~\cite{parkes2015economic}. Many strategies, solutions, and thoughts have been shared surrounding these canonical problems. However, as identified by Leibo et al.~\cite{leibo2017multi}, \emph{real-world} dilemmas are ``temporally extended''---that is, require dynamic policies over time, and are hence \emph{sequential}. This additional element makes these dilemmas far less tractable.

To demonstrate how such difficulties can be overcome, Leibo et al.~\cite{leibo2017multi} approached two temporally-extended dilemmas, by adopting a multi-agent RL solution. Interestingly, in doing so, the researchers were able to infer the nature of conflict and competition in the said dilemmas, thereby gaining insight into their real-world analogues. Herein we notice a slightly different advantage of RL in agent-based simulations: not only do they free us of having to hard-code the agents' behaviours, we can moreover gain interesting insights into the emergent dynamics that arise. Of course, such benefits are inherently impossible when using a hard-coded approach, since we cannot gain insights into something we are defining \emph{a priori}. We see, then, yet another way that \emph{learning} has the potential to benefit agent-based modelling in computational economics.

